Real-time Visual Object Tracking with Natural Language Description

In recent years, deep-learning-based visual object trackers have been studied thoroughly, but handling occlusions and/or rapid motion of the target remains challenging. In this work, we argue that conditioning on the natural language (NL) description of a target provides information for longer-term invariance, and thus helps cope with typical tracking challenges. However, deriving a formulation to combine the strengths of appearance-based tracking with the language modality is not straightforward. We propose a novel deep tracking-by-detection formulation that can take advantage of NL descriptions. Regions that are related to the given NL description are generated by a proposal network during the detection phase of the tracker. Our LSTM based tracker then predicts the update of the target from regions proposed by the NL based detection phase. In benchmarks, our method is competitive with state of the art trackers, while it outperforms all other trackers on targets with unambiguous and precise language annotations. It also beats the state-of-the-art NL tracker when initializing without a bounding box. Our method runs at over 30 fps on a single GPU.

==> figures/fig-detection-phase.tex <==
\begin{figure*}
    \begin{center}
        \begin{equation*}
            \left.
            \begin{array}{l}
                I_t \xrightarrow{\text{CNN}} F_t \xrightarrow[\text{RoI Pooling}]{\text{RPN}} \mathbf{X}_t, \mathbf{RF}_t \\
                Q
            \end{array}
            \right\}
            \xrightarrow[\text{Network}]{\text{Language}}
            \mathbf{S}_t, \mathbf{X}_t, \mathbf{RF}_t
            \xrightarrow[\mathbf{S}_t]{\text{Top-}N}
            \mathbf{X}_t^\text{det}, \mathbf{RF}_t^\text{det}
        \end{equation*}
        \caption{Architecture of the detection module. Output bounding boxes \(\mathbf{X}_t^\text{det}\) and their corresponding regional convolution
            features \(\mathbf{RF}_t^\text{det}\)
            chosen by the RPN and the language network are passed into the tracking module.}
        \label{fig-detection-phase}
        \vspace{-0.3in}
    \end{center}
\end{figure*}


==> figures/fig-intermediate-box.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/rpn-result.png}
    \caption{Bounding boxes proposed by \(F_\text{RPN}\).}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/lang-result.png}
    \caption{Top-5 bounding boxes from \(F_\text{lang}\).}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/gt.png}
    \caption{Ground truth bounding box.}
    \label{fig-otb-success-performance}
  \end{subfigure}
  \caption{Intermediate bounding boxes proposed by RPN \(\mathbf{X}_t^\text{RPN}\) , and top-5 bounding boxes from Language network \(\mathbf{X}_t^\text{lang}\), together with corresponding ground truth bounding box \(X_t^*\). Query \(Q\) is \text{kite flying in the sky}.}
  \label{fig-intermediate-box}
\end{figure*}


==> tables/tbl-lang-performance.tex <==
\begin{table}
\begin{center}
  \begin{tabular}{lcccc}
    \hline
    &\multicolumn{2}{c}{\textbf{OTB}} &\multicolumn{2}{c}{\textbf{LaSOT}}  \\
    \textbf{Tracker} & Suc. & Prec. & Suc. & Prec.  \\
    \hline
    Ours (Box+NL)& 0.61 & 0.79 & 0.35 & 0.35\\
    Li~\cite{Li} (Box+NL) & 0.55 & 0.72 & - & -\\
    \hline
    Ours (NL Only) & 0.54 & 0.78 & 0.28 & 0.28\\
    Li~\cite{Li} (NL Only) & 0.25 & 0.29 & - & -\\
    \hline
  \end{tabular}
  \caption{Comparison between best published NL based tracker Li~\cite{Li},
    and our proposed tracker on LaSOT and OTB-99-lang with different set-ups.
    AUC of success plots and precision plots (shown in Fig.~\ref{fig-performance}
    and Fig.~\ref{fig-nl-tracker}) are reported. As~\cite{Li} only released
    code for OTB dataset, LaSOT results are omitted in this table.  Box+NL
    stands for models that condition on both NL and ground truth bounding box
    at frame 1. NL-Only stands for models that condition only on NL.}
  \label{tbl-lang-performance}
\end{center}
\end{table}


==> tables/tbl-resets.tex <==
\begin{table*}
    \begin{center}
        \begin{tabular}{c|c|c|c|c}
            \hline
            Video & Proposed Tracker & ECO & Model I \cite{Li} & \(\cdots\) \\
            \hline
            Overall & 3.5/5.4/7.7/3.1 & 4.0/5.0/5.0/- & 5.0/5.0/5.0/5.0 & \(\cdots\) \\
            \hline
            Doll & 3/5/7/3 & 4/5/5/- & 5/5/5/5 & \(\cdots\) \\
            \hline
            Ball-1 & 3/5/7/3 & 4/5/5/- & 5/5/5/5 & \(\cdots\) \\
            \hline
        \end{tabular}
    \end{center}
    \caption{Placeholder:Number of resets need for each tracker, different threshold (0/0.1/0.3/(0 but reset with language only)). \newline \textbf{Fabricated Data. DO NOT USE IN SUBMISSION.}}
    \label{tbl-resets}
\end{table*}

